Graph Traversal with Tensor Functionals: A Meta-Algorithm for Scalable Learning

Graph Representation Learning (GRL) methods have impacted fields from chemistry to social science. However, their algorithmic implementations are specialized to specific use-cases e.g.message passing methods are run differently from node embedding ones. Despite their apparent differences, all these methods utilize the graph structure, and therefore, their learning can be approximated with stochastic graph traversals. We propose Graph Traversal via Tensor Functionals(GTTF), a unifying meta-algorithm framework for easing the implementation of diverse graph algorithms and enabling transparent and efficient scaling to large graphs. GTTF is founded upon a data structure (stored as a sparse tensor) and a stochastic graph traversal algorithm (described using tensor operations). The algorithm is a functional that accept two functions, and can be specialized to obtain a variety of GRL models and objectives, simply by changing those two functions. We show for a wide class of methods, our algorithm learns in an unbiased fashion and, in expectation, approximates the learning as if the specialized implementations were run directly. With these capabilities, we scale otherwise non-scalable methods to set state-of-the-art on large graph datasets while being more efficient than existing GRL libraries - with only a handful of lines of code for each method specialization. GTTF and its various GRL implementations are on: https://github.com/isi-usc-edu/gttf.

==> proof_generalization.tex <==
\subsection{Proof of Proposition \ref{prop:augment} under assumptions}
We show that Proposition 8 holds under the following assumptions:
(i) the graph is $\alpha$-regular random, (ii) and connected. (iii) Data is whitened: $X^\top X = I$. (iv) There are many edges: $f \ll \alpha$.
The model we consider is one layer GCN with linear activation, (v) trained to reduce squared Frobenius norm error. Assumption (v) was also assumed by  \cite{dropout2014baldi} for analyzing the effect of Dropout.
Assumption (i) makes the analysis easier. If assumption (ii) was violated, our analysis will still apply with a modification that the number of models would be $\mathcal{O}(\sum_g (n_g)^{binom{\alpha}{f}})$ where the sum $g$ is taken over connected components and $n_g$ is the number of nodes in subgraph $g$. Assumption (iii) is usually met by data whitening or applying BatchNorm at the input. Assumption (iv) motivates our method (if there are only a few edges, perhaps the need for sampling is obviated).  The model we consider is given by:
\[
H(A, X; W)  =  \accentset{\circ}{A} X W \scalebox{0.8}{$\textrm{ \ \ \ with \ \ \ } 
\accentset{\circ}{A} = D^{'-1/2} A^{'} D^{'-1/2};
D' = \textrm{diag}( A' \vec{\mathbf{1}}_n); \ \  A' = \max(A, A^\top) + I_{n\times n}$}
\]
where the symmetric normalization $\accentset{\circ}{A}$, appeared in \citep{kipf}, yields $\accentset{\circ}{A}^\top = \accentset{\circ}{A}$.
%This form works for directed graphs (with asymmetric $A$) and is used by GraphSAGE.
% B. McKay and N. Wormald, "Uniform Generation of Random Regular Graphs of Moderate Degree," Journal of Algorithms, Vol. 11 (1990)



Given an $\alpha$-regular graph, invoking \textit{Traverse} with $B=V$ (all nodes) and $F=[f]$ (i.e. depth $=1$) will choose $f$ edges, uniformly at random, from $\alpha$ choices, for each node. Since there are $\binom{\alpha}{f}$ choices for each node, then there are $n^{\binom{\alpha}{f}}$ sampled adjacency matrices. We now define a 
set
\begin{equation}
\mathcal{A} = \{ A_c \}_{c=1}^{|\mathcal{A}|}
%; \textrm{ \ \ \  \  \ \ \  \  each with  \ \ \  \  \ \ \  \  }   \textrm{diag}(A_c \vec{\mathbf{1}}_n)^{-1} = \frac{1}{f} I_{n \times n}
\end{equation}
where $|\mathcal{A}| = n^{\binom{\alpha}{f}}$.
Note that for each $A_c$ contains $f$ non-zeros in every row, and since the graph is large, random, and regular, then it also contains $\approx$$f$ non-zeros in every column. Applying normalization $\circ$, proposed by \citep{kipf}, gives matrix $\accentset{\circ}{A}_c$ with $\approx$~$2f+1$ non-zeros in each row.
Further, let $z \sim \textrm{Categorical}\left(\frac{1}{|\mathcal{A}|},  \frac{1}{|\mathcal{A}|}, \dots, \frac{1}{|\mathcal{A}|} \right)$,
which we
define as Multinoulli distribution as a selector over the elements of $\mathcal{A}$.
Each sampled $z$ will have one of its entries to 1 and all others to zero. This allows us analyze GTTF's behavior. 
Specifically,
%
%$p_1, p_2, \dots, p_{|\mathcal{A}|} = 1$
%
%Further, we define a probability distribution over elements of $\mathcal{A}$ that is uniform: $P(\mathcal{A}) = \frac{1}{|\mathcal{A}|}$.
%With these,
running GTTF with \textsc{\texttt{RootedAdjAcc}}  (defined in Eq.~\ref{eq:rootedAdjAcc}) then passing the accumulated adjacency to $H$ will output:
\begin{equation}
H_\mathcal{F} \triangleq \sum_{c=1}^{|\mathcal{A}|} z_c   H(A_c, X; W) 
%=  \textrm{diag}(\widetilde{A} \vec{\mathbf{1}}_n)^{-1} \widetilde{A} X W
= \frac{1}{f}  \sum_{c=1}^{|\mathcal{A}|} z_c  \accentset{\circ}{A}_c X W \textrm{ \ \ \ with \ \ \ } z \sim \textrm{Categorical}\Bigg(\overbrace{\frac{1}{|\mathcal{A}|},  \frac{1}{|\mathcal{A}|}, \dots, \frac{1}{|\mathcal{A}|}}^{|\mathcal{A}| \textrm{ of them}} \Bigg)
\end{equation}
Now consider, consider training $|\mathcal{A}|$ models, one model per adjacency $A_c \in \mathcal{A}$. Let
\begin{equation}
H_c \triangleq H(A_c, X; W_c).
\end{equation}
For regression against label matrix $Y$ (with rows containing continuous targets for nodes), one can minimize:
\begin{equation}
\min_{W_c} \frac{1}{2} || Y - H_c ||_F^2 =  \min_{W_c} \frac{1}{2} ||Y - \accentset{\circ}{A}_c X W_c||_F^2,
\end{equation}
obtains a closed-form minimizer $W_c^* = (\accentset{\circ}{A}_c X)^+ Y$, where $(.)^+$ denotes Moore-Penrose inverse and $||.||_F$ denotes Frobenius norm. Expanding and applying our assumptions:
\begin{align}
W_c^* &= (\accentset{\circ}{A}_c X)^+ Y = (X^\top \overbrace{\accentset{\circ}{A}_c \accentset{\circ}{A}_c}^{\scalebox{.8}{$ \begin{array}{c} \textrm{\tiny{Assump. (iv)}} \\  \approx \frac{1}{(2f+1) } I_{n \times n} \end{array} $}}  X)^{-1} X^\top \accentset{\circ}{A}_c   Y \nonumber \\
& \approx (2f+1) (\underbrace{X^\top X}_{\scalebox{.8}{$ \begin{array}{c} = I \\ \textrm{\tiny{Assump. (iii)}}  \end{array} $}} )^{-1} X^\top \accentset{\circ}{A}_c   Y \nonumber \\
&= (2f+1) X^\top \accentset{\circ}{A}_c   Y
\end{align}
The product $\accentset{\circ}{A}_c \accentset{\circ}{A}_c$ counts the number of mutual neighbors in each entry: since we are sampling from a large graph, the mutual connections between any two nodes will be close to $\approx 0$ but the mutual connections of a node with itself (i.e. the diagonal $\accentset{\circ}{A}_c \accentset{\circ}{A}_c$) is $= \frac{1}{(2f+1)}$ given the symmetric renormalization trick. An Ensemble model ($H_\textrm{ENS}$), averaging all trained $H_c$'s is equivalent to averaging $W_c$'s as $H$ is linear in $W$. Specifically:
\[
H_\textrm{ENS}(A, X) \triangleq  H\left( A, X; \frac{1}{|\mathcal{A}|} \sum_{c} W_c^*\right),
\]
with $W^*_\textrm{ENS} = \frac{1}{|\mathcal{A}|} \sum_{c} W_c^*$. Showing $\frac{\partial}{\partial W} \mathds{E}[\frac12 || Y - H_\mathcal{F}||_F^2 ] \Big\vert_{W^*_\textrm{ENS}} = 0$, implies that our method converges to, and therefore equivalent to, a model averaging all $n^{\binom{\alpha}{f}}$ models, concluding our proof.
\begin{align*}
\frac{\partial}{\partial W} &\mathds{E}\Big[\frac12 || Y - H_\mathcal{F}||_F^2 \Big] = \mathds{E}\Big[ \big(\sum_c z_c X^\top \accentset{\circ}{A}_c \big) \big(\sum_c z_c \accentset{\circ}{A}_c X  \big) W \Big] - \mathds{E}\Big[ \big(\sum_c z_c X^\top \accentset{\circ}{A}_c \big) Y \Big] \\
& = \mathds{E}\Big[ X^\top \big(\big[\sum_c \underbrace{\left( z_c \right)^2}_{\textrm{(indicator) =$z_c$ }} \underbrace{\accentset{\circ}{A}_c^\top \accentset{\circ}{A}_c}_{\ \ \approx \frac{1}{(2f+1) } I} \big] + \big[\sum_{c \neq l}  \underbrace{z_c z_l}_{\textrm{ (exclusive) =0}} \accentset{\circ}{A}_c^\top \accentset{\circ}{A}_l \big]   \big) X W \Big] - \mathds{E}\Big[ \big(\sum_c z_c X^\top \accentset{\circ}{A}_c \big) Y \Big] \\
& \approx \frac{1}{(2f+1)} \mathds{E}\Big[ X^\top \big(\underbrace{\big[\sum_c z_c  \big]}_{=1}    \big) X W \Big] -  \big( \sum_c \mathds{E}[z_c] X^\top \accentset{\circ}{A}_c \big) Y  \\
&=  \frac{1}{(2f+1)} W - \frac{1}{|\mathcal{A}|} \sum_c X^\top \accentset{\circ}{A}_c Y.
\end{align*}
Finally, plugging into the above $W=W^*_\textrm{ENS} = \frac{1}{|\mathcal{A}|} \sum_{c} W_c^* = \frac{1}{|\mathcal{A}|} \sum_{c} (2f+1) X^\top \accentset{\circ}{A}_c Y$, gives 0. $\square$





% \begin{prop}
%     For general graph convolution methods, under the assumption of a convex objective function, using GTTF results in unbiased learning. In other words, if $\theta^*$ is the global minimum of the loss function $g(\theta)$, then gradient descent on $g$ converges to $\theta^*$.
% \end{prop}

% The assumption of convexity has been used consistently across many previous works, such as FastGCN \citep{fastgcn} and GraphSaint \citep{graphsaint-iclr2020}.
% The full proof of this can also be found in the supplementary material. 

% \begin{proof}
%     Let $\sigma(\accentset{\circ}{A}^kH^{(l-1)}W^{(l)})$ be the general one layer activation function of a graph convolution model. If $\sigma$ is linear then, the multi-layer activation becomes $\boldsymbol{H} = S\accentset{\circ}{A}^k...\accentset{\circ}{A}^kXW^{(1)}...W^{(L)}$, where $L$ is the number of layers. The expectation of the output is:
%     \[\mathds{E}\left[ S\accentset{\circ}{A}^k...\accentset{\circ}{A}^kXW^{(1)}...W^{(L)} \right]=S\mathds{E}\left[\accentset{\circ}{A}^{kL}\right]XW^{(1)}...W^{(L)}\]
%     By Prop 4, this is unbiased as long as kL is within the context distance of the random walks. Let $\boldsymbol{h}$ be the output vector for classifying a single node.
    
%     Under the most common classification objective, cross-entropy, the loss gradient is $\nabla\left(-\left<\boldsymbol{y},\log{(\text{softmax}(\boldsymbol{h}}))\right>\right)$, where $y$ is the one-hot label. \textcolor{red}{Having issues with softmax cross-entropy}
    
    
    
    
% \end{proof}


%\subsection{Complexity Analysis}

%\textcolor{red}{Move ``Note on scale'' to here. Mention GCN complexity as $O(\min(|E|, f^h))$}

%\begin{enumerate}
 %   \item Space Complexity - The space complexity of our algorithm is $\mathcal{O}(sizeof(A') + sizeof(\delta) + sizeof(\Omega)) = \mathcal{O}(|E| +|V| + |B|f^{C}) = \mathcal{O}(|E|)$. This is linear in the size of the graph. %In contrast, \citet{abu-wys}, the approach that we build off of, is quadratic in the size of the graph since it requires storing $\mathcal{T}^k$ in memory.
    
 %   \item Time Complexity - The time complexity of generating the random walk forest $\Omega$ for a batch is $\mathcal{O}(|B|f^{C})$. This gives our approach a total time complexity of $\mathcal{O}(|V|f^{C})$ for an entire epoch i.e. linear in the size of the graph. %This is significantly better than \citet{abu-wys}'s complexity of $\mathcal{O}(|V|^3k)$ to compute $\mathcal{T}^k$. 
%\end{enumerate}


% \section{MapReduce for CompactAdj}

% \begin{algorithm}
%   \DontPrintSemicolon
%   \SetKwFunction{FMap}{Map}
%   \SetKwFunction{FReduce}{Reduce}
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FMap{$edge$}}{
%     $(u, v) \gets edge$\;
%     emit($u$, $v$)\;
%     emit($v$, $u$)\;
%   }
%   \;
%   \SetKwProg{Pn}{Function}{:}{\KwRet}
%   \Fn{\FReduce{$node$, $neighbors$}}{%
%     $degree \gets 0$\;
%     \ForEach{$v \in neighbors$}{%
%         $CompactAdjIndices\texttt{.push}([node,degree])$\;
%         $CompactAdjValues\texttt{.push}(v)$\;
%         $degree \gets degree + 1$\;
%         emit($"A"$, $(node, degree)$, $v$)\;
%     }
%     emit($"D"$, $node$, $degree$)\;
%   }
% \caption{MapReduce for CompactAdj}
% \label{algorithm:mapreduce}
% \end{algorithm}

